Generative Long-form Question Answering: Relevance, Faithfulness and Succinctness

In this thesis, we investigated the relevance, faithfulness, and succinctness aspects of Long Form Question Answering (LFQA). LFQA aims to generate an in-depth, paragraph-length answer for a given question, to help bridge the gap between real scenarios and the existing open-domain QA models which can only extract short-span answers. LFQA is quite challenging and under-explored. Few works have been done to build an effective LFQA system. It is even more challenging to generate a good-quality long-form answer relevant to the query and faithful to facts, since a considerable amount of redundant, complementary, or contradictory information will be contained in the retrieved documents. Moreover, no prior work has been investigated to generate succinct answers. We are among the first to research the LFQA task. We pioneered the research direction to improve the answer quality in terms of 1) query-relevance, 2) answer faithfulness, and 3) answer succinctness.

==> 2_authorization.tex <==
\null\skip0.2in
\begin{center}
{\bf \Large \underline{Authorization}}
\end{center}
\vspace{12mm}

I hereby declare that I am the sole author of the thesis.

\vspace{10mm}

I authorize the Hong Kong University of Science and Technology to lend this
thesis to other institutions or individuals for the purpose of scholarly research.

\vspace{10mm}

I further authorize the Hong Kong University of Science and Technology to
reproduce the thesis by photocopying or by other means, in total or in part, at the
request of other institutions or individuals for the purpose of scholarly research.

\vspace{30mm}

\begin{center}
\underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}\\
~~~~\thesisauthor \\
~~~~\signdate

\end{center}


==> 3_signature.tex <==
\begin{center}
{\Large \thesistitle}\\
\vspace{5mm}
by\\
\vspace{3mm}
\thesisauthor\\
\vspace{5mm}
This is to certify that I have examined the above PhD thesis\\
and have found that it is complete and satisfactory in all respects,\\
and that any and all revisions required by\\
the thesis examination committee have been made.
\end{center}

\vspace{12mm}

\begin{center}
\underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ }\\
\supervisorinfo
\end{center}

% \vspace{15mm}
% \begin{center}
% \underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ }\\
% \cosupervisorinfo
% \end{center}

\vspace{12mm}
\begin{center}
\underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ }\\
\depheadinfo
\end{center}

\vspace{4mm}

\textbf{Thesis Examination Committee}
\TabPositions{5cm}
\begin{enumerate}[itemsep=-4.0mm]
    \item Prof. Pascale Fung \tab Department of Electronic and Computer Engineering
    \item Prof. Bertram Shi \tab Department of Electronic and Computer Engineering
    \item Prof. Qifeng Chen \tab Department of Electronic and Computer Engineering
    \item Prof. Lei Chen  \tab Department of Computer Science and Engineering
    % \item Prof. David Cheng Chang \tab Department of Humanities
    \item Prof. Heng Ji \tab Department of Computer Science, University of Illinois at Urbana-Champaign
\end{enumerate}


\vspace{5mm}
\begin{center}
\departmentname\\
\vspace{1mm}
\signdate
\end{center}


==> 4_dedicate.tex <==
\thispagestyle{empty}
\null\vskip0.5in
\begin{center}


  \vspace{20mm}

  \begin{LARGE}
    \dedicate
  \end{LARGE}

  \vspace{4mm}
 hello world!


\end{center}

\vfill


==> 5_acknowledgement.tex <==
\centerline{{\bf \Large Acknowledgments}} \vspace{5mm} \noindent

Firstly, I would like to express my most sincere gratitude to my supervisor, Professor Pascale Fung, for her knowledgeable guidance and supervision throughout my Ph.D. The valuable research opportunities she suggested, such as the 'Chatbot Millionaire Challenge' and 'Kaggle COVID-19 Open Research Dataset Challenge', have triggered my research interest and led to my research outcomes on question answering. Furthermore, her confidence in me and continuous support for my research work have inspired me to push myself to achieve huge impacts and made my Ph.D. journey less lonely. Furthermore, her excellent research taste, which I have been learning from, allowed me to grow constantly as a researcher. Also, as my role model, her passionate and positive attitude in life and work has affected my mindset and helped me conquer many difficulties. 

Next, I would like to express my appreciation to Professor Bertram Shi, Professor Qifeng Chen, Professor Lei Chen, and Professor Heng Ji for taking their time to be on my thesis examining committee. I am also thankful to Professor Bertram Shi and Professor Qifeng Chen for being on my thesis proposal committee and providing me with insightful feedback. I also want to thank Tania Leigh Wilmshurst, who proofread my papers many times and gave me insightful and useful advice on academic writing.

In the last four years, I have had an exciting journey in the CAiRE lab with amazing lab colleagues. Therefore, I want to thank Yan Xu, Tiezheng Yu, Peng Xu, Elham Barezi and Farhad Bin Siddique, Ziwei Ji, Wenliang Dai, and Zihan Liu for the past collaborations. My thanks go to Yan Xu for the collaborations on my early stage question answering projects, including the 'Chatbot Millionaire Challenge' and 'Kaggle COVID-19 Open Research Dataset Challenge'; it is a great pleasure to work with her; to Tiezheng Yu for the multiple great collaborations on summarization research and on the World Health Organization(WHO) projects; to Peng Xu for the insightful discussions on question generation projects; to Elham Barezi and Farhad Bin Siddique for the support on 'Kaggle COVID-19' projects; to Zihan Liu for discussions on the prompting based context generation work; and to Wenliang Dai and Ziwei Ji for their help on the multi-hop question generation paper. Thanks also go to Andrea Madotto, Zhaojiang Lin, and Genta Winata, who provided useful suggestions at the beginning of my Ph.D., and to Samuel Cahyawijaya, Yejin Bang, Etsuko Ishii, Nayoen Lee, and many others for the invaluable research experiences. 

I would further like to express my thanks to Dr. Xin Jiang, Xiaoguang Li, Dr. Lifeng Shang, and Professor Qun Liu, from Huawei Noah's Ark AI Lab, for the valuable research discussions and insightful feedback on the long-form question-answering projects during my internship there; their passion at research and their research attitude also affected me. I would like to thank Dr. Mostofa Patwary, Dr. Shrimai Prabhumoye, Dr. Peng Xu, Dr. Ryan Prenger, Dr. Mohammad Shoeybi, and Prof. Anima Anandkumar, and Bryan Catanzaro for their time, support and significant research interactions during my internship at Nvidia ADLR group. The insightful discussions on weekly meetings on my project with the whole group, and personal meetings with Mohammad every week, have helped improve my research habits and enhanced my research skills. 

Finally, I would like to express my gratitude to my friends in Shenzhen and Hong Kong, who have motivated me during the challenging times. The WeChat chatting during the COVID-19 pandemic and the relaxed Friday night dinner moment has given me unforgettable memories. I want to give my deepest appreciation to my family for supporting me all the way during my Ph.D., especially to my 3-years old niece 'little candy' who has brought so much happiness to me with her pure and innocent smile. Last but not least, I would like to thank my boyfriend, Dr. Jindi Zhang, for the quality time together and for his support all the time.

==> abstract_backup.tex <==
%!TEX program = xelatex
%!TEX root = ./thesis.tex
\begin{center}
{\Large \textbf{\thesistitle}}\\
\vspace{20mm}
by \thesisauthor\\
%\vspace{15mm}
\departmentname\\
%\vspace{10mm}
The Hong Kong University of Science and Technology
\end{center}
\vspace{8mm}
\begin{center}
\Large Abstract
\end{center}
\par
\noindent

\setlength{\emergencystretch}{10pt}

Question answering (QA) aims to build computer systems that can automatically answer questions posed by humans, and has been a long-standing problem in natural language processing(NLP). This thesis investigates the particular problem of generative long-form question answering (\textbf{LFQA}), which aims to \textbf{generate} an in-depth, paragraph-length answer for a given question posed by a human. 

Generative LFQA is an important task. Many of the everyday questions that humans deal with and pose to search engines require multi-sentence explanations, for example, \textit{How do jellyfish function without a brain?} \textit{Why wouldn't life on another habitable planet look similar to Earth's?} or \textit{What are the risking factors related to COVID-19?}. However, conventional work on QA is mainly extractive, which means a short and concise span is extracted from a passage as the answer. These systems are thus incompetent at answering non-trivial questions. Thus, LFQA is needed to provide complete and accurate answers to complex questions.

However, LFQA is under-explored compared to the extractive QA task, and it is more challenging. Multiple documents containing tens of thousands of tokens must be synthesized to provide the answer, which is difficult for the generation model to handle. Furthermore, since a considerable amount of redundant, complementary, or contradictory information will be contained in the retrieved documents, how to generate a good-quality long-form answer that is grammatically correct and semantically informative is even more challenging. 

In this thesis, we investigate the task of LFQA and tackle the aforementioned challenges. Specifically, we focus on 1) how to build a practical application for real-time open-domain LFQA, and generate query-relevant answers, 2) how to generate fact-aware long-form answers, and 3) how to leverage the informative generated long-form answers.

To elaborate, we firstly present a real-time LFQA system which can generate multiple-documents-based answers efficiently. The system demonstrates its effectiveness at generating fluent and somewhat relevant answers, winning one of the Kaggle competitions related to COVID-19. And we propose to incorporate the explicit answer relevance of the source documents into the generation model to enhance the relevance of the generated answer. 

Secondly, we present a new end-to-end framework for generative QA that jointly models answer generation and machine reading to tackle the answer faithfulness challenge. State-of-the-art results on two LFQA datasets demonstrate the effectiveness of our method in comparison with strong baselines on automatic and human evaluation metrics. The method also topped one public leaderboard on the LFQA task. 

Finally, we propose a simple yet effective framework for \textit{closed-book} question answering (QA), which directly answer an open-domain question without access to any external knowledge. We leverage the generated long-form answers as the intermediate bridge between the huge amount of parameterized knowledge stored in pretrained language models and short answer. Experimental results on three QA benchmarks show that our method significantly outperforms previous \textit{closed-book} QA methods and is par with traditional \textit{open-book} methods that exploit external knowledge source.


% In this thesis, we investigate the task of LFQA and tackle the aforementioned challenges. Specifically, we first investigate how we can build a practical application for real-time open-domain LFQA. Then, we focus on enhancing the answer quality, in terms of 1) \textbf{fluency}, i.e., grammatical correctness, and low repetition, 2) \textbf{relevance} to the answer, and 3) \textbf{faithfulness}, which measures the factual correctness of the generated answer.

% We first present a real-time LFQA system which can generate multiple-documents-based answers efficiently. The system also demonstrates its effectiveness at generating fluent and somewhat relevant answers, winning one of the Kaggle competitions related to COVID-19. Then, we propose to incorporate the explicit answer relevance of the source documents into the generation model to enhance the relevance of the generated answer. Finally, we present a new end-to-end framework for generative QA that jointly models answer generation and machine reading to tackle the answer faithfulness challenge. State-of-the-art results on two LFQA datasets demonstrate the effectiveness of our method in comparison with strong baselines on automatic and human evaluation metrics. The method also topped one public leaderboard on the LFQA task.







==> achievements.tex <==
\null\skip0.2in
\begin{center}
{\bf \Large \underline{Competition Awards}}
\end{center}
\vspace{12mm}
% (* denotes equal contribution)
\begin{enumerate}[leftmargin=*]

\item {Asian Dean's Forum 2022 – The Rising Stars Women in Engineering Workshop} \hfill {2022}
\\ \textit{shortlisted participant} (https://risingstarsasia.org/index.php)

\item {2nd Dial2Doc Workshop \textbf{Best Student Paper Award}} \hfill {2022}
\\"Retrieval-Free Knowledge-Grounded Dialogue Response Generation with Adapters". 
\\Yan XU, Etsuko, Samuel Cahyawijaya, Zihan Liu, Genta Indra, Andrea Madotto, \textbf{Dan Su}, Pascale Fung

 \item {\textbf{Top-1} on KILT Leaderboard} \hfill {2021}
% \\ "Read before Generate! Faithful Long Form Question Answering with Machine Reading".
\\KILT is a public leaderboard organized by researchers from Facebook AI, for knowledge intensive NLP tasks.
 \\\textbf{Leaderboard Top-1} on the open-domain QA task. (\textbf{1-person team})
\\(\url{https://eval.ai/web/challenges/challenge-page/689/leaderboard/1908}).

\item {\textbf{Top-1} on Computational Linguistics Lay Summary Challenge
} \hfill {2020}\\
% \\\textbf{1st place winner}. \\
"Dimsum @LaySumm 20: BART-based Approach for Scientific Document Summarization" \\
(\url{https://competitions.codalab.org/competitions/25516#participate})

\item {\textbf{1st Place Winner} Kaggle COVID-19 Open Research Dataset Challenge (\href{https://www.kaggle.com/allen-institute-for-ai/CORD-19-research-challenge/tasks}{CORD-19})} \hfill {2020}
\\An AI challenge organized by AllenAI, Chan Zuckerberg Initiative, The White House ect. \\\textbf{1st place winner} (\textbf{team leader}) on task 10, out of > 500 international teams, received \$1000 from the organizer.
(\url{https://www.kaggle.com/datasets/allen-institute-for-ai/CORD-19-research-challenge/discussion/148807})
 \item {\textbf{1st Place Winner} Chatbot Millionaire Challenge} \hfill 2019
\\In "AI+U: Explore and Experience Exhibition", organized by Hong Kong Science \& Technology Park. 
\\\textbf{1st place winner} (\textbf{team leader}), received a prize of HK\$30,000.
(\url{https://www.hkstp.org/press-room/hkstp-s-aiplusu-explore-and-
experience-exhibition-brings-together-the-ai-community-to-charter-next-path-of-growth/})

 \item {Machine Reading for Question Answering (MRQA) 2019 Shared Task} \hfill 2019
\\Ranked \textbf{4/10} among all, including industry competitors like Baidu Inc.(1st), Apple Inc.(2nd). (\textbf{team leader})

\end{enumerate}



==> chapter1_backup.tex <==
\chapter{Introduction}


%%% maybe a paragraph


\section{Open-domain Question Answering}

Open domain question answering (ODQA) has been a long-standing problem in the history of NLP~\cite{simmons1964indexing,kupiec1993murax,voorhees1999trec,moldovan2000structure, harabagiu2000experiments, brill2002analysis, ferrucci2010building, baudivs2015yodaqa, lin2003question,gliozzo2012natural, yih2016question, sachan2018standardized, chen2017reading}. The goal of open domain question answering is to build automated computer systems which are able to answer any sort of (factoid) questions that humans might ask, based on a large collection of unstructured natural language documents, structured data, semi-structured data or even other modalities such as images or videos (as illustrated in Figure~\ref{fig:intro_odqa}). 
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/intro/intro_odqa.pdf}
  \caption{A Open-domain question answering system illustration. The text-based QA is the most extensively studied ODQA task.}
  \label{fig:intro_odqa}
\end{figure}

\textbf{Text-based QA} The most extensively studied ODQA task is \textit{text-based} QA, which derives an answer from unstructured natural language documents (e.g., encyclopedias, dictionaries, news articles, and general Web documents). 
Dating back to the 1960s~\cite{simmons1964indexing}, the text-based open-domain question answering(QA) has been broadly investigated by both the information retrieval (IR) and natural language processing (NLP) communities  ~\cite{simmons1964indexing,kupiec1993murax,voorhees1999trec,moldovan2000structure, harabagiu2000experiments, brill2002analysis, ferrucci2010building, baudivs2015yodaqa, lin2003question,gliozzo2012natural, yih2016question, sachan2018standardized, chen2017reading, su2020improving}. Notable text-based QA systems include Microsoft’s ASKMSR~\cite{brill2002analysis}, IBM’s DEEPQA~\cite{ferrucci2010building}, and DrQA~\cite{chen2017reading}. 

\textbf{Extractive open-domain QA}  Almost all of the previous \textit{text-based} ODQA systems are \textbf{extractive}-based~\cite{chen2017reading,izacard2021leveraging, lewis2021paq}, which means they extract a short and concise span from a retrieved document as the answer, as the example in Figure~\ref{fig:intro_extractive_qa} illustrated. Normally the extractive ODQA can provide factoid information for simple straightforward, factual queries such as \textit{Which artist sings this song?} , \textit{Who is the president of the US?}, or \textit{Where is HKUST located?}.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/intro/intro_extractive_QA.png}
  \caption{An extractive, text-based open-domain QA system illustration.}
  \label{fig:intro_extractive_qa}
\end{figure}

\section{Generative Long-form Question Answering}
While the \textbf{extractive} open-domain QA task have been extensively studied in prior years, the \textbf{generative} open-domain QA that tries to generate an answer for a given question obtains little attention. 
To fill the blank and further push the field forward, the more challenging task, long-form question answering (LFQA) was recently proposed~\cite{fan2019eli5}. 

LFQA aims to \textbf{generate} an in-depth, paragraph-length answer for a given question. The questions are more complicated such as the \textit{why/how} type questions, that requires in-depth explanations. They can’t be directly answered by short-phrase span or sentences from existing documents. Instead, they normally requires to synthesize information from multiple web documents comprising hundreds of thousands of words, identifying the relevant information in those documents, and using world knowledge to answer. We show an LFQA examples in Table~\ref{tab:intro_lfqa_example}. As we can see, it require multiple sentences to explain the answer for the given question, and the long-form answers are generated from multiple documents and using world knowledge.

\begin{table}[htb!]
    \centering
    \begin{adjustbox}{width={0.9\textwidth},totalheight={\textheight},keepaspectratio}
\begin{tabular}{p{1\columnwidth}}
    \hline
    % \hline
% \textbf{Question:} Which  French ace pilot and adventurer fly L'Oiseau Blanc?  \\
% \textbf{Short answer}: Charles Eugène \\
% \textbf{Long answer}:  On May 8, 1927, \textbf{Charles Nungesser} and Francois Coli boarded L'Oiseau blanc, a 450-hp Lorraine-powered Levasseur biplane designed to compete for the Orteig Prize. They took off from Paris on 8 May 1927 and were last seen over Ireland. Less than two weeks later, Charles Lindbergh successfully made the New York-Paris journey and claimed the prize in the Spirit of St. Louis. \\
% \hline
\textbf{Question:} How do Jellyfish function without brains or nervous systems? \\
\textbf{Answer:} Jellyfish may not have a brain, but they have a rough
nervous system and innate behaviours. However, they are
very simple creatures. They’re invertebrate: creatures without
a backbone. Most jellyfish have really short life spans.
Sometimes just a couple of hours. [...] As their name implies,
they are largely composed of basically jelly inside a
thin membrane. They’re over 95\% water. (327 words) \\
    \hline
    % \hline
    \end{tabular}
    % }
\end{adjustbox}
\caption{Generative long-form question answering example. The example is from the “Explain Like I’m Five” (ELI5)~\cite{fan2019eli5}.}
\label{tab:intro_lfqa_example}
\end{table}

%  The first question is from the HotpotQA dataset~\cite{yang2018HotpotQA}, seeking information for a multi-hop question. As we can see, the extractive QA system tries to extract a short precise answer, the generative-based LFQA aims to generate a long answer. The multi-sentence long answer gives a detailed explanation, which could be used to understand and verify the short answer. 

\section{Motivation}
% Building automated computer systems to answer questions asked by humans in natural language is one of the most elusive and long-standing challenges in the history of artificial intelligence. While we are thrilled at the achievements the community has made~\cite{brill2002analysis, ferrucci2010building, chen2017reading}, the current textual-based ODQA systems have limitations. Almost all of the previous ODQA systems are \textbf{extractive}-based, they can only provide factoid information for simple queries, such as the \textit{who/when/where} type questions, and are incompetent at answering non-trivial questions such as \textit{How do jellyfish function without a brain?}, \textit{Why wouldn't life on another habitable planet look similar to Earth's?}, or \textit{What are the risking factors related to COVID-19?}. However, a large ratio of the questions that humans pose to search engines every day are those complicated types, and require multi-sentence, in-depth explanations. Therefore, it motivates us to work on the newly-proposed, more challenging LFQA task.


Building automated computer systems to answer questions asked by humans in natural language is one of the most elusive and long-standing challenges in the history of artificial intelligence. While we are thrilled at the achievements the community has made~\cite{brill2002analysis, ferrucci2010building, chen2017reading}, the current textual-based ODQA systems can not answer non-trivial questions such as the \textit{why/how} type ones. This is because almost all of the previous ODQA systems are \textbf{extractive}-based, which will extract short-span based phrases from retrieved document as the answer, so they can only provide factoid information for simple queries, such as the \textit{who/when/where} type questions. However, a large ratio of the questions that humans pose to search engines every day are those complicated types, such as \textit{How do jellyfish function without a brain?}, \textit{Why wouldn't life on another habitable planet look similar to Earth's?}, or \textit{What are the risking factors related to COVID-19?}, there is no short answer and require multi-sentence, in-depth explanations. Therefore, it motivates us to work on the newly-proposed, more challenging LFQA task.

LFQA have many possible applications. It could be integrated to facilitate a more intelligent search engine ~\cite{metzler2021rethinking}. For example, if we search Google with a query, it could not only returns a list of search documents but also attempts to read these Web documents and even display some generated answers at the top of the search results. Additionally, LFQA could play an important role in digital personal assistants systems such as Amazon's ALEXA, Apple's SIRI, GOOGLE ASSISTANT, to enhance user experience. As it has been shown\footnote{\tt \small https://voicebot.ai/2019/03/12/smart-speaker-owners-agree-that-questions\\-music-and-weather-are-killer-apps-what-comes-next/smart-speaker-use-case-\\frequency-january-2019-01/}, \textit{'asking a question'} is the most frequently used functions from those smart speakers. Specifically, it might be used to generate explanations as a complement to short phrase answers for factoid information-seeking open-domain questions~\cite{kwiatkowski2019natural, yang2018hotpotqa}, or to answer open-ended questions like the ones from the Reddit forum "Explain Like I'm Five"~\cite{fan2019eli5}. 

\begin{table}[!ht]
\centering
\begin{adjustbox}{width={0.99\textwidth},totalheight={0.9\textheight},keepaspectratio}
\begin{tabular}{p{1\columnwidth}}
\hline
\textbf{Question:} what does abc stand for in liquor store? \\
\textbf{Generated Answer:} \hlgreen{\textbf{A liquor store} is a retail shop that predominantly sells prepackaged alcoholic beverages intended to be consumed off the store's premises. Depending on region and local idiom (social issue), they may also be called bottle store, off licence, (in United Kingdom, Ireland, and New Zealand) bottle shop, bottle-o package store, party store (in Michigan), ABC store, state store, or other similar terms.}\\
\textbf{Golden Answer:} Most of these states have an \textbf{Alcoholic Beverage Control (ABC)} board and run liquor stores called ABC stores. In all monopoly states a parallel license system is used to regulate the sale and distribution of lighter alcoholic beverages such as beer and wine.\\
\hline
\end{tabular}
\end{adjustbox}
\caption{Example from the MSMARCO dataset~\cite{nguyen2016ms}. The generated answer gives a detailed definition and introduction of 'liquor store', however, it doesn't answer the representation of 'abc'. Therefore, the answer lacks of \textbf{relevance} to the given question. We highlight in green the sentences \hlgreen{irrelevant} to the question.}
\label{tab:intro_challenge_examples_1}
\end{table}

\begin{table}[!ht]
\centering
\begin{adjustbox}{width={0.99\textwidth},totalheight={0.9\textheight},keepaspectratio}
\begin{tabular}{p{1\columnwidth}}
\hline
\textbf{Question:} definition of sadduction \\
\textbf{Generated Answer:} Sadducees. noun. \hlred{The definition of a sadducee is a person who acts in a deceitful or duplicitous manner.  An example of a Sadduceee is a politician who acts deceitfully in order to gain political power}. 1 a member of a Jewish sect that was active during the Second Temple. \\
\textbf{Golden Answer:} The Sadducees(Hebrew: \d{S}ĕdûqîm) were a sect or group of Jews that were active in Judea during the Second Temple period, starting from the second century BCE through the destruction of the Temple in 70 CE. The sect was identified by Josephus with the upper social and economic ecoshon of Judean society.\\
 \hline
\end{tabular}
\end{adjustbox}
\caption{Example from the MSMARCO dataset~\cite{nguyen2016ms}. The answer is hallucinated and lacks of \textbf{faithfulness}. We mark in red the \hlred{unfaithful} snippets.}
\label{tab:intro_challenge_examples_2}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{adjustbox}{width={0.92\textwidth},totalheight={0.9\textheight},keepaspectratio}
\begin{tabular}{p{1\columnwidth}}
    \hline
\textbf{Question:} Which  French ace pilot and adventurer fly L'Oiseau Blanc?  \\
\textbf{Short answer}: Charles Eugène \\
\textbf{Long answer}:  On May 8, 1927, \textbf{Charles Nungesser} and Francois Coli boarded L'Oiseau blanc, a 450-hp Lorraine-powered Levasseur biplane designed to compete for the Orteig Prize. They took off from Paris on 8 May 1927 and were last seen over Ireland. Less than two weeks later, Charles Lindbergh successfully made the New York-Paris journey and claimed the prize in the Spirit of St. Louis. \\
\hline
    \end{tabular}
    % }
\end{adjustbox}
\caption{The generated long-form answer provides context information and can be used to extract the short answer. The example is from the “Explain Like I’m Five” (ELI5)~\cite{fan2019eli5}.}
\label{tab:intro_challenge_example_3}
\end{table}

\section{Research Directions}

LFQA is a newly proposed, more challenging task compared to the traditional extractive-based open-domain QA, and little work has yet been done on it.

In this thesis, we study methods to build and improve a LFQA system. Specifically, we focus on:
\begin{itemize}
    \item \textbf{Generating query-relevant long-form answers} In recent years, we have witnessed rapid progress in dense retrieval techniques like REALM~\cite{guu2020realm}, DPR~\cite{karpukhin2020dense} and ORQA~\cite{lee2019latent}. Also, the large pre-trained language models~\cite{lewis2020bart,raffel2020exploring} have demonstrated its superior performances at many generation tasks such as summerization~\cite{su2021improve,yu2020dimsum}, question generation~\cite{su2022qa4qg,su2020multi}. However, few work have been investigated to build an effective real-time LFQA system. Since LFQA is quite a challenging task that requires more than just concatenating the two techniques. Firstly, it needs to handle the issue of applying pre-trained language model which has limited input sequence length, to process the multiple relevant documents containing more than thousand of tokens for generation. Secondly, those multiple retrieved documents may include irrelevant, complementary or contradictory information, how to generate more query-relevant, long-form answers is another challenge (we show an example in Table~\ref{tab:intro_challenge_examples_1} to provide a better understanding). Therefore, we first propose CAiRE-COVID, a real-time long form question answering system for COVID-19, which combines information retrieval with state-of-the-art QA and query-focused multi-document summarization techniques, to answer high priority COVID-19 related questions. Then, we introduce QFS-BART, a model that incorporates the explicit answer relevance of the source documents given a query into the answer generation model, to generate more query-relevant answers.
    
    % Fluency is the first important evaluation element in many generation tasks, such as abstractive summarization~\cite{su2021improve}, text generation~\cite{su2020multi,su2022read}. It measures the linguistic quality of the generated text. If a long-form answer that is not fluent, such as containing repetitions or grammatical incorrect statements, it will harm the answer contents greatly. 
    
    % Furthermore, the generated answer should contain information that is relevant to the topic of the question. We show an example in Table~\ref{tab:intro_challenge_examples_1} to provide a better understanding. The generated answer gives a detailed definition and introduction of 'liquor store' in a fluent way, however, it lacks \textbf{query-relevance} since the information does not answer the question: \textit{'What does abc stand for?'}. 

    % Therefore, how to generate fluent, query-relevant long-form answers is an important task to build an effective LFQA system.

    \item \textbf{Generating fact-aware long-form answers} Improving the fact correctness of the generated answer is one of the other main challenges for LFQA task~\cite{krishna2021hurdles, lin2021truthfulqa, nakano2021webgpt}. Specifically, the generated answer should be faithful to facts in the souce documents~\cite{ji2022survey}. In the example in Table~\ref{tab:intro_challenge_examples_2}, the answer is fluent, and also relevant to the query when trying to elaborate the \textit{'definition of sadduction'}. However, the content itself is hallucinated and lacks \textbf{faithfulness}. Such a fluent and relevant but unfaithful answer will mislead the user. Therefore, we propose an end-to-end framework named RBG, to augment the generation model with fine-grained, answer-related salient information predicted by an machine reading comphrehension(MRC) module, to improve and generate fact-aware answer that is more faithful to the source documents.
    
    \item \textbf{Leveraging informative long-form answers}
    % As illustrated in Figure~\ref{fig:intro_extractive_qa}, a traditional open-domain QA system normally retrieves multiple relevant contexts from an external knowledge corpus, then it extracts a short answer span from the retrieved contexts as the answer. While the generative long-form answers contains informative statements relevant to a given question, it might be leveraged as replacement of the retrieved contexts for extractive ODQA task (An concrete example is shown in~\ref{tab:intro_challenge_example_3}). No prior work has been investigated on this. 
    \textit{Closed-book} question answering (QA) requires a model to directly answer an open-domain question without access to any external knowledge~\cite{roberts2020much}. While it has been shown that large pretrained LMs store abundant knowledge~\cite{petroni2019language,roberts2020much}, prior work do not fully exploit the stored knowledge to answer the question~\cite{roberts2020much, ye2020studying,brown2020language, radford2019language}. Therefore, to address this issue and further improve the accuracy of \textit{closed-book} QA model, we propose a simple yet effective framework named \textbf{CGAP} for open-domain QA, by leveraging the generated long-form answers as the intermediate bridge between the huge amount of parameterized knowledge and short answer (we show an example in Table~\ref{tab:intro_challenge_example_3}). CGAP performs \textbf{C}ontext \textbf{G}eneration followed by \textbf{A}nswer \textbf{P}rediction via two-stage prompting using large pretrained LMs. Experimental results on three QA benchmarks show that our method significantly outperforms previous \textit{closed-book} QA methods and is par with traditional \textit{open-book} methods that  exploit external knowledge source.

\end{itemize}

\section{Thesis Outline}
The thesis is divided in four main chapters, plus a conclusion. It is organized as:
\begin{itemize}
    \item Chapter 2 first gives an overview of open-domain question answering. Then we will introduce the preliminaries needed throughout the thesis for generative QA, followed by the related work to LFQA. 
    \item Chapter 3 have two parts. The first part presents CAiRE-COVID. A real-time LFQA system which can generate multiple-documents-based answers efficiently. The system demonstrates its effectiveness at generating fluent and somehow relevant answers, winning one of the Kaggle competitions related to COVID-19. The second part presents QFS-BART, a model that incorporates the explicit answer relevance of the source documents given a query, via a MRC model, into the BART model, to generate coherent and more query-relevant answer. 
    \item Chapter 4 presents RBG, a new end-to-end framework that jointly models answer generation and machine reading to augment the generation model with fine-grained, answer-relevant salient information from each retrieved documents, as an emphasis on faithful facts, to improve the answer faithfulness. 
    \item Chapter 5 introduces CGAP, a first of its kind system that leverage the generated long-form answers as the context, for open-domain question answering.
\end{itemize}


% State-of-the-art results on two LFQA datasets demonstrate the effectiveness of our method, in comparison with strong baselines on automatic and human evaluation metrics. The method also topped one public leaderboard on the LFQA task.







==> conclusion_backup.tex <==
\chapter{Conclusion}

In this thesis, we study methods to build and improve a LFQA system. Specifically, we focus on: how to build a real-time LFQA system and generate more query-relevant answers, how to generate fact-aware long-form answers, and how to leverage the informative generated long-form answers.

In generating query-relevant long-form answers, we first present CAiRE-COVID, a real-time long form question answering system for COVID-19, which combines information retrieval with state-of-the-art QA and query-focused multi-document summarization techniques, to answer high priority COVID-19 related questions. Then, we introduce QFS-BART, a model that incorporates the explicit answer relevance of the source documents given a query into the answer generation model, to generate more query-relevant answers. CAiRE-COVID has won one of the 10 tasks in the Kaggle COVID-19 Open Research Dataset Challenge\footnote{\tt \small  https://www.kaggle.com/allen-institute-for-ai/CORD-19-research-challenge}, by generating relevant and fluent answers to salient COVID-19 related questions, judged by medical experts. QFS-BART obtains state-of-the-art results on query-focused summarization dataset. 

In generating fact-aware long-form answers, we propose an end-to-end framework named RBG (\textbf{r}ead \textbf{b}efore \textbf{g}enerate) to improve and generate fact-aware answer that is more faithful to the source documents. The main idea is to augment the generation model with fine-grained, answer-related salient information predicted by an machine reading comphrehension(MRC) module. State-of-the-art results on two LFQA datasets demonstrate the effectiveness of our method, in comparison with strong baselines on automatic and human evaluation metrics. The method also topped one public leaderboard~\footnote{\tt \small https://evalai.cloudcv.org/web/challenges/challenge-page/689/leaderboard/1908} on the LFQA task.

In leveraging generated long-form answers for extractive open-domain QA task, we propose to leverage generated long-form answers as the intermediate bridge between the huge amount of parameterized knowledge in large pretrained LMs and the answer for closed-book QA(CBQA), which directly answer the open-domain questions without access to any external knowledge sources, and leverages the parametric knowledge stored in large pretrained language models (LMs)~\cite{raffel2020exploring, brown2020language, ye2020studying}. To the best of our knowledge, no previous investigation has been conducted on generating long-form answers from large pretrained LMs for CBQA and leveraging them to predict answer. Experimental results on three QA benchmarks show that our method significantly outperforms previous \textit{closed-book} QA methods (e.g. exact matching 68.6\% vs. 55.3\%), and is on par with \textit{open-book} methods that exploit external knowledge sources (e.g. 68.6\% vs. 68.0\%). Our method is able to better exploit the stored knowledge in pretrained LMs without adding extra learnable parameters or needing finetuning, and paves the way for hybrid models that integrate pretrained LMs with external knowledge.

% Overall
In future work, we expect to develop LFQA systems that can provide more query-relevant and fact-aware answers, and also generalize well on updated new facts. In fact, in the three chapters of this thesis, we open new exciting research directions for LFQA system: 1) there are still possible ways worth to explore to build more query-relevant LFQA system. In Chapter 3, we try to improve query-relevance via the QFS task, while the quality of the relevant document retrieved from external corpus also affects the generation model. In future works, more sophisticated retrieval techniques such as iterative retrieval should be explored on the task. 2) building a fact-aware LFQA system is still in its infancy. In Chapter 4, we leverage a machine reading comprehension model to highlight the salient information in the retrieved documents. While combining other knowledge modalities such as the knowledge bases (KBs), or visual materials etc. to provide more informative and diverse knowledge, might also help improve the factual of the generated answer. 3) leverage the generated long-form answers might further help other tasks. In Chapter 5, we explored it's possibility to help improve open-domain QA. Actually the generated long-form answers could also be used as intermediate evidences on a reasoning task.

% discussion about retrieval system for LFQA, like iterative retrieval. blablabla. (2) faithfulness evaluation metrics, and datasets. (3) new-domain.. (4) with multiple knowledge sources...(5) human in the loop, reinforcemenet learning, to learn and evolve. (since some questions might be no forever correct answer, the answer could (6) explicitly reasoning process (since currently it is more like just information synthesis, but lacks real reasoning)..



==> publication.tex <==
\null\skip0.2in
\begin{center}
{\bf \Large \underline{List of Publications}}
\end{center}
\vspace{12mm}
% (* denotes equal contribution)
\begin{enumerate}[leftmargin=*]
    \item \textbf{Dan Su}, Mostofa Patwary, Shrimai Prabhumoye, Peng Xu, Ryan Prenger, Mohammad Shoeybi, Pascale Fung, Anima Anandkumar, Bryan Catanzaro, \textit{"Context Generation Improves Open Domain Question Answering"}, submitted to \textbf{EMNLP2022}
    
   \item Yejin Bang, Nayeon Lee, Tiezheng Yu, Leila Khalatbari, Yan Xu, \textbf{Dan Su}, Elham J. Barezi, Andrea Madotto, Hayden Kee, Pascale Fung, \textit{"AISOCRATES: Towards Answering Ethical Quandary Questions"}, [under submission to EMNLP 2022]
    
    \item Ziwei Ji, Nayeon Lee, Rita, Tiezheng Yu, \textbf{Dan Su}, Yan Xu, Etsuko Ishii, Yejin Bang, Andrea Madotto, Pascale Fung, \textit{"Survey of Hallucination in Natural Language Generation"}, [under submission to ACM Computing Surveys]
    
    \item Wenliang Dai, Zihan Liu, Ziwei Ji, \textbf{Dan Su}, Pascale Fung, \textit{Plausible May Not Be Faithful: Probing Object Hallucination in Vision-Language Pre-training}, [under submission to EMNLP 2022]

    \item \textbf{Dan Su}, Xiaoguang Li, Jindi Zhang, Xin Jiang, Lifeng Shang, Qun Liu, Pascale Fung, \textit{"Read before Generate! Faithful Long Form Question Answering with Machine Reading"}, 60th Annual Meeting of the Association for Computational Linguistics \textbf{[ACL 2022]}
    \item \textbf{Dan Su}, Peng Xu, Pascale Fung, \textit{"QA4QG: Using Question Answering to Constrain Multi-Hop Question Generation"}, 2022 IEEE International Conference on Acoustics, Speech and Signal Processing \textbf{[ICASSP 2022]}
    \item Yan XU, Etsuko, Samuel Cahyawijaya, Zihan Liu, Genta Indra, Andrea Madotto, \textbf{Dan Su}, Pascale Fung, \textit{"Retrieval-Free Knowledge-Grounded Dialogue Response Generation with Adapters"}, 2nd DialDoc Workshop at ACL 2022, Online, 22-27 May 2022 \textbf{[DialDoc Best Student Paper Award]}
    \item LOVENIA Holy; etc.,\textbf{Dan Su}, Pascale Fung, \textit{"Clozer: Adaptable Data Augmentation for Cloze-style Reading Comprehension"}, Repl4NLP 2022 (ACL Workshop), Dublin, Ireland, 26 May 2022. \textbf{[ACL 2022]}
    \item Pascale Fung, \textbf{Dan Su}, T. Yu, Y. Xu, Y. Yang, P. AbdelMalik, J. Schnitzler, T. Cornelissen, D. Milovanovic, \textit{"Improving Public Health Surveillance using Automatic Summarization"}, The European Scientific Conference on Applied Infectious Disease Epidemiology \textbf{[ESCAIDE 2021]}
    \item \textbf{Dan Su}, Tiezheng Yu, Pascale Fung, \textit{"Improve Query Focused Abstractive Summarization by Incorporating Answer Relevance"}, Findings of the Association for Computational Linguistics: ACL 2021 \textbf{[ACL 2021]}
    \item \textbf{Dan Su}, Yan Xu, Tiezheng Yu, Farhad Bin Siddique, Elham J Barezi, Pascale Fung, \textit{"CAiRE-COVID: A Question Answering and Query-focused Multi-Document Summarization System for COVID-19 Scholarly Information Management"}, Proceedings of the 1st Workshop on NLP for COVID-19 (also accepted as EMNLP Demo paper) \textbf{[EMNLP 2020]}
    \item \textbf{Dan Su}, Yan Xu, Wenliang Dai, Ziwei Ji, Tiezheng Yu, Pascale Fung, \textit{"Multi-hop Question Generation with Graph Convolutional Network"}, Findings of the Association for Computational Linguistics: EMNLP 2020 \textbf{[EMNLP 2020]}
    
    \item  Tiezheng Yu, \textbf{Dan Su}, Wenliang Dai, Pascale Fung, \textit{Dimsum @LaySumm 20: BART-based Approach for Scientific Document Summarization"}, Proceedings of the First Workshop on Scholarly Document Processing \textbf{[EMNLP 2020]}
    \item \textbf{Dan Su} and Pascale Fung, \textit{"Improving Spoken Question Answering Using Contextualized Word Representation"}, 2020 IEEE International Conference on Acoustics, Speech and Signal Processing \textbf{[ICASSP 2020]}
    \item \textbf{Dan Su}, Yan Xu, Genta Indra Winata, Peng Xu, Hyeondey Kim, Zihan Liu, Pascale Fung, \textit{"Generalizing Question Answering System with Pre-trained Language Model Fine-tuning"}, In Proceedings of the 2nd Workshop on Machine Reading for Question Answering \textbf{[EMNLP 2019]}
    \item \textbf{Dan Su}, Pascale Fung, Nicolas Auguin, \textit{"Multimodal Music Emotion Classification Using AdaBoost with Decision Stumps"}, 2013 IEEE International Conference on Acoustics, Speech and Signal Processing \textbf{[ICASSP 2013]}
    \item \textbf{Dan Su}, Pascale Fung, \textit{"These Words are Music to my Ears: Recognizing Music Emotion from Lyrics Using AdaBoost"}, 2013 Asia-Pacific Signal and Information Processing Association Annual Summit and Conference
     \textbf{[APSIPA ASC 2013]}
    \item \textbf{Dan Su}, Pascale Fung, \textit{"Personalized Music Emotion Classification via Active Learning"}, Proceedings of the Second International ACM Workshop on Music Information Retrieval with User-centered and Multimodal Strategies \textbf{[ACMMM 2012]}
\end{enumerate}


